A C-Band Fully Polarimetric Automotive Synthetic Aperture Radar

Due to the rapid increase in 76 GHz automotive spectrum use in recent years, wireless interference is becoming a legitimate area of concern. However, the recent rise in interest of automated vehicles (AVs) has also spurred new growth and adoption of low frequency vehicle-to-everything (V2X) communications in and around the 5.8 GHz unlicensed bands, opening the possibility for communications spectrum reuse in the form of joint radar-communications (JRC). In this work, we present a low frequency 5.9 GHz side-looking polarimetric synthetic aperture radar (SAR) for automotive use, utilizing a ranging waveform in a common low frequency V2X communications band. A synthetic aperture technique is employed to address the angular resolution concerns commonly associated with radars at lower frequencies. Three side-looking fully polarimetric SAR images in various urban scenes are presented and discussed to highlight the unique opportunities for landmark inference afforded through measurement of co- and cross-polarized scattering.

==> Rev 1.2 (FINAL) - arXiv/acronyms.tex <==
% --- Acronyms ------------------------

% Signals/Signal Processing
\DeclareAcronym{lfm}{
	short = LFM,
	long = linear frequency modulation
}
\DeclareAcronym{prf}{
	short = PRF,
	long = pulse repetition frequency
}
\DeclareAcronym{pri}{
	short = PRI,
	long = pulse repetition interval
}
\DeclareAcronym{fmcw}{
	short = FMCW,
	long = frequency modulated continuous-wave
}
\DeclareAcronym{lfmcw}{
	short = LFMCW,
	long = linear frequency modulated continuous-wave
}
\DeclareAcronym{cw}{
	short = CW,
	long = continuous-wave
}
\DeclareAcronym{dbf}{
	short = DBF,
	long = digital beamforming
}
\DeclareAcronym{sar}{
	short = SAR,
	long = synthetic aperture radar
}
\DeclareAcronym{psr}{
	short = PSR,
	long = point scatterer response
}
\DeclareAcronym{rcs}{
	short = RCS,
	long = radar cross-section
}
\DeclareAcronym{crlb}{
	short = CRLB,
	long = Cramer-Rao lower bound
}
\DeclareAcronym{dof}{
	short = DoF,
	long = degree of freedom
}
\DeclareAcronym{snr}{
	short = SNR,
	long = signal-to-noise ratio
}
\DeclareAcronym{sinr}{
	short = SINR,
	long = signal-to-interference-plus-noise ratio
}
\DeclareAcronym{fft}{
	short = FFT,
	long = fast Fourier transform,
}
\DeclareAcronym{ifft}{
	short = IFFT,
	long = inverse \ac{fft},
}
\DeclareAcronym{ift}{
	short = IFT,
	long = inverse Fourier transform,
}
\DeclareAcronym{rmse}{
	short = RMSE,
	long = root-mean-square error
}
\DeclareAcronym{psd}{
	short = PSD,
	long = power spectral density
}
\DeclareAcronym{rca}{
	short = RCA,
	long = range of closest approach
}
\DeclareAcronym{rda}{
	short = RDA,
	long = Range-Doppler Algorithm
}
\DeclareAcronym{rma}{
	short = RMA,
	long = Range Migration Algorithm
}
\DeclareAcronym{pfa}{
	short = PFA,
	long = Polar Formatting Algorithm
}
\DeclareAcronym{bpa}{
	short = BPA,
	long = Backprojection Algorithm
}
\DeclareAcronym{rvp}{
	short = RVP,
	long = residual video phase
}
\DeclareAcronym{jrc}{
	short = JRC,
	long = joint radar-communications
}
\DeclareAcronym{doa}{
	short = DOA,
	long = direction of arrival
}
\DeclareAcronym{hci}{
	short = HCI,
	long = human-computer interaction
}
\DeclareAcronym{its}{
	short = ITS,
	long = intelligent transportation systems
}
\DeclareAcronym{rtk}{
	short = RTK,
	long = real-time kinematic
}
\DeclareAcronym{eirp}{
	short = EIRP,
	long = effective isotropic radiated power
}
\DeclareAcronym{gnss}{
	short = GNSS,
	long = global navigation satellite system
}
\DeclareAcronym{imu}{
	short = IMU,
	long = inertial measurement unit
}


% Communications
\DeclareAcronym{ofdm}{
	short = OFDM,
	long = orthogonal frequency division multiplexing
}


% Hardware
\DeclareAcronym{pll}{
	short = PLL,
	long = phase-locked loop
}
\DeclareAcronym{vco}{
	short = VCO,
	long = voltage-controlled oscillator
}
\DeclareAcronym{lna}{
	short = LNA,
	long = low-noise amplifier
}
\DeclareAcronym{if}{
	short = IF,
	long = intermediate frequency
}
\DeclareAcronym{cots}{
	short = COTS,
	long = commercial off-the-shelf
}
\DeclareAcronym{adc}{
	short = ADC,
	long = analog to digital converter
}
\DeclareAcronym{lo}{
	short = LO,
	long = local oscillator
}
\DeclareAcronym{pcb}{
	short = PCB,
	long = printed circuit board
}
\DeclareAcronym{mimo}{
	short = MIMO,
	long = multiple-input multiple-output
}
\DeclareAcronym{simo}{
	short = SIMO,
	long = single-input multiple-output
}
\DeclareAcronym{mmic}{
	short = MMIC,
	long = monolithic microwave integrated circuit
}
\DeclareAcronym{daq}{
	short = DAQ,
	long = data acquisition
}
\DeclareAcronym{ic}{
	short = IC,
	long = integrated circuit
}
\DeclareAcronym{pa}{
	short = PA,
	long = power amplifier
}



% Company acronyms
\DeclareAcronym{ti}{
	short = TI,
	long = Texas Instruments
}
\DeclareAcronym{adi}{
	short = ADI,
	long = Analog Devices
}


% Misc.
\DeclareAcronym{roi}{
	short = ROI,
	long = region of interest,
	long-plural-form = regions of interest
}
\DeclareAcronym{v2x}{
	short = V2X,
	long = vehicle-to-everything
}
\DeclareAcronym{av}{
	short = AV,
	long = automated vehicle
}
\DeclareAcronym{cors}{
	short = CORS,
	long = continuously operating reference station
}
\DeclareAcronym{mdot}{
	short = MDOT,
	long = Michigan Department of Transportation
}
\DeclareAcronym{moco}{
	short = MOCO,
	long = motion compensation
}



